Solar synthetic imaging: Introducing denoising diffusion probabilistic models on SDO/AIA data

Given the rarity of significant solar flares compared to smaller ones, training effective machine learning models for solar activity forecasting is challenging due to insufficient data. This study proposes using generative deep learning models, specifically a Denoising Diffusion Probabilistic Model (DDPM), to create synthetic images of solar phenomena, including flares of varying intensities. By employing a dataset from the AIA instrument aboard the SDO spacecraft, focusing on the 171 {\AA} band that captures various solar activities, and classifying images with GOES X-ray measurements based on flare intensity, we aim to address the data scarcity issue. The DDPM's performance is evaluated using cluster metrics, Frechet Inception Distance (FID), and F1-score, showcasing promising results in generating realistic solar imagery. We conduct two experiments: one to train a supervised classifier for event identification and another for basic flare prediction, demonstrating the value of synthetic data in managing imbalanced datasets. This research underscores the potential of DDPMs in solar data analysis and forecasting, suggesting further exploration into their capabilities for solar flare prediction and application in other deep learning and physical tasks.

==> references.tex <==
@article{ho2020,
  author    = {Jonathan Ho and
               Ajay Jain and
               Pieter Abbeel},
  title     = {Denoising Diffusion Probabilistic Models},
  journal   = {CoRR},
  volume    = {abs/2006.11239},
  year      = {2020},
  url       = {https://arxiv.org/abs/2006.11239},
  eprinttype = {arXiv},
  eprint    = {2006.11239},
  timestamp = {Tue, 23 Jun 2020 17:57:22 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2006-11239.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@misc{ho2022classifierfree,
      title={Classifier-Free Diffusion Guidance}, 
      author={Jonathan Ho and Tim Salimans},
      year={2022},
      eprint={2207.12598},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@article{sohldick,
  author    = {Jascha Sohl{-}Dickstein and
               Eric A. Weiss and
               Niru Maheswaranathan and
               Surya Ganguli},
  title     = {Deep Unsupervised Learning using Nonequilibrium Thermodynamics},
  journal   = {CoRR},
  volume    = {abs/1503.03585},
  year      = {2015},
  url       = {http://arxiv.org/abs/1503.03585},
  eprinttype = {arXiv},
  eprint    = {1503.03585},
  timestamp = {Mon, 13 Aug 2018 16:47:30 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/Sohl-DicksteinW15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{classifierguidance,
  author    = {Prafulla Dhariwal and
               Alex Nichol},
  title     = {Diffusion Models Beat GANs on Image Synthesis},
  journal   = {CoRR},
  volume    = {abs/2105.05233},
  year      = {2021},
  url       = {https://arxiv.org/abs/2105.05233},
  eprinttype = {arXiv},
  eprint    = {2105.05233},
  timestamp = {Fri, 14 May 2021 12:13:30 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2105-05233.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{Galvez_2019,
	doi = {10.3847/1538-4365/ab1005},
  
	url = {https://doi.org/10.3847%2F1538-4365%2Fab1005},
  
	year = 2019,
	month = {may},
  
	publisher = {American Astronomical Society},
  
	volume = {242},
  
	number = {1},
  
	pages = {7},
  
	author = {Richard Galvez and David F. Fouhey and Meng Jin and Alexandre Szenicer and Andr{\'{e}
}s Mu{\~{n}}oz-Jaramillo and Mark C. M. Cheung and Paul J. Wright and Monica G. Bobra and Yang Liu and James Mason and Rajat Thomas},
  
	title = {A Machine-learning Data Set Prepared from the {NASA} Solar Dynamics Observatory Mission},
  
	journal = {The Astrophysical Journal Supplement Series}
}

@ARTICLE{aia,
       author = {{Lemen}, James R. and {Title}, Alan M. and {Akin}, David J. and {Boerner}, Paul F. and {Chou}, Catherine and {Drake}, Jerry F. and {Duncan}, Dexter W. and {Edwards}, Christopher G. and {Friedlaender}, Frank M. and {Heyman}, Gary F. and {Hurlburt}, Neal E. and {Katz}, Noah L. and {Kushner}, Gary D. and {Levay}, Michael and {Lindgren}, Russell W. and {Mathur}, Dnyanesh P. and {McFeaters}, Edward L. and {Mitchell}, Sarah and {Rehse}, Roger A. and {Schrijver}, Carolus J. and {Springer}, Larry A. and {Stern}, Robert A. and {Tarbell}, Theodore D. and {Wuelser}, Jean-Pierre and {Wolfson}, C. Jacob and {Yanari}, Carl and {Bookbinder}, Jay A. and {Cheimets}, Peter N. and {Caldwell}, David and {Deluca}, Edward E. and {Gates}, Richard and {Golub}, Leon and {Park}, Sang and {Podgorski}, William A. and {Bush}, Rock I. and {Scherrer}, Philip H. and {Gummin}, Mark A. and {Smith}, Peter and {Auker}, Gary and {Jerram}, Paul and {Pool}, Peter and {Soufli}, Regina and {Windt}, David L. and {Beardsley}, Sarah and {Clapp}, Matthew and {Lang}, James and {Waltham}, Nicholas},
        title = "{The Atmospheric Imaging Assembly (AIA) on the Solar Dynamics Observatory (SDO)}",
      journal = {\solphys},
     keywords = {Solar corona, Solar instrumentation, Solar imaging, Extreme ultraviolet},
         year = 2012,
        month = jan,
       volume = {275},
       number = {1-2},
        pages = {17-40},
          doi = {10.1007/s11207-011-9776-8},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012SoPh..275...17L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sunpy,
  doi = {10.3847/1538-4357/ab4f7a},
  url = {https://iopscience.iop.org/article/10.3847/1538-4357/ab4f7a},
  author = {{The SunPy Community} and Barnes, Will T. and Bobra, Monica G. and Christe, Steven D. and Freij, Nabil and Hayes, Laura A. and Ireland, Jack and Mumford, Stuart and Perez-Suarez, David and Ryan, Daniel F. and Shih, Albert Y. and Chanda, Prateek and Glogowski, Kolja and Hewett, Russell and Hughitt, V. Keith and Hill, Andrew and Hiware, Kaustubh and Inglis, Andrew and Kirk, Michael S. F. and Konge, Sudarshan and Mason, James Paul and Maloney, Shane Anthony and Murray, Sophie A. and Panda, Asish and Park, Jongyeob and Pereira, Tiago M. D. and Reardon, Kevin and Savage, Sabrina and Sipőcz, Brigitta M. and Stansby, David and Jain, Yash and Taylor, Garrison and Yadav, Tannmay and Rajul and Dang, Trung Kien},
  title = {The SunPy Project: Open Source Development and Status of the Version 1.0 Core Package},
  journal = {The Astrophysical Journal},
  volume = {890},
  issue = {1},
  pages = {68-},
  publisher = {American Astronomical Society},
  year = {2020}
}

@misc{noaa_goes_solar_flare,
  author = {NOAA},
  title = {GOES Solar Flare Classification},
  year = {2023},
  url = {https://www.swpc.noaa.gov/products/goes-x-ray-flux},
  note = {Accessed: [access date]}
}

@article{HEK,
	doi = {10.1007/s11207-010-9624-2},
  
	url = {https://doi.org/10.1007%2Fs11207-010-9624-2},
  
	year = 2010,
	month = {dec},
  
	publisher = {Springer Science and Business Media {LLC}
},
  
	volume = {275},
  
	number = {1-2},
  
	pages = {67--78},
  
	author = {N. Hurlburt and M. Cheung and C. Schrijver and L. Chang and S. Freeland and S. Green and C. Heck and A. Jaffey and A. Kobashi and D. Schiff and J. Serafin and R. Seguin and G. Slater and A. Somani and R. Timmons},
  
	title = {Heliophysics Event Knowledgebase for~the~Solar Dynamics Observatory ({SDO}) and Beyond},
  
	journal = {Solar Physics}
}

@article{hackstein2023,
title = {Evaluation metrics for galaxy image generators},
journal = {Astronomy and Computing},
volume = {42},
pages = {100685},
year = {2023},
issn = {2213-1337},
doi = {https://doi.org/10.1016/j.ascom.2022.100685},
url = {https://www.sciencedirect.com/science/article/pii/S2213133722000993},
author = {S. Hackstein and V. Kinakh and C. Bailer and M. Melchior},
keywords = {Deep learning, Generative models, Computer-vision, Evaluation, Galaxy morphology},
abstract = {A major problem with deep generative models is verifying that the generated distribution resembles the target distribution while the individual generated sample is indistinguishable from the original data. In particular, for application in astrophysics we need to be sure that the generated data matches our prior knowledge and that the generated samples entail all object types with the correct frequency and diversity. We currently lack objective ways to systematically assess these quality aspects, where human inspection reaches its limits, as this requires detailed analysis of a large data volume. In this work, we identify reasonable metrics for the quality of galaxy image generators. To this end, we compare a small set of conditional image generators, trained on galaxy images with classification labels for visual morphology features. Our main contribution is a new set of cluster-based metrics for matching the generated distribution to the target distribution. Furthermore, we use the Wasserstein distance on proxies for galaxy morphology as well as a number of other metrics commonly used for image generators. The newly introduced cluster-based metrics are good proxies for the quality of the generated distribution and are suited for automatized identification of mode collapse. Furthermore, the cluster metrics allow for a qualitative interpretation of the generated distribution. The metrics based on morphological statistics provide a useful tool to probe the physical soundness of generated samples. Finally, we find that kernel inception distance used with an InceptionV3 model pre-trained on ImageNet is a good proxy for the overall quality of galaxy image generators, although it cannot be interpreted that easily.}
}

@article{FID,
  author    = {Martin Heusel and
               Hubert Ramsauer and
               Thomas Unterthiner and
               Bernhard Nessler and
               G{\"{u}}nter Klambauer and
               Sepp Hochreiter},
  title     = {GANs Trained by a Two Time-Scale Update Rule Converge to a Nash Equilibrium},
  journal   = {CoRR},
  volume    = {abs/1706.08500},
  year      = {2017},
  url       = {http://arxiv.org/abs/1706.08500},
  eprinttype = {arXiv},
  eprint    = {1706.08500},
  timestamp = {Sat, 23 Jan 2021 01:20:58 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/HeuselRUNKH17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{f1score,
 ISSN = {00359246},
 URL = {http://www.jstor.org/stable/2984875},
 abstract = {A broadly applicable algorithm for computing maximum likelihood estimates from incomplete data is presented at various levels of generality. Theory showing the monotone behaviour of the likelihood and convergence of the algorithm is derived. Many examples are sketched, including missing value situations, applications to grouped, censored or truncated data, finite mixture models, variance component estimation, hyperparameter estimation, iteratively reweighted least squares and factor analysis.},
 author = {A. P. Dempster and N. M. Laird and D. B. Rubin},
 journal = {Journal of the Royal Statistical Society. Series B (Methodological)},
 number = {1},
 pages = {1--38},
 publisher = {[Royal Statistical Society, Wiley]},
 title = {Maximum Likelihood from Incomplete Data via the EM Algorithm},
 urldate = {2023-04-12},
 volume = {39},
 year = {1977}
}

@misc{sakurai2022,
      title={Probability Distribution Functions of Solar and Stellar Flares}, 
      author={Takashi Sakurai},
      year={2022},
      eprint={2212.02678},
      archivePrefix={arXiv},
      primaryClass={astro-ph.SR}
}

@misc{ramesh2022,
      title={Hierarchical Text-Conditional Image Generation with CLIP Latents}, 
      author={Aditya Ramesh and Prafulla Dhariwal and Alex Nichol and Casey Chu and Mark Chen},
      year={2022},
      eprint={2204.06125},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@misc{ronneberger2015unet,
      title={U-Net: Convolutional Networks for Biomedical Image Segmentation}, 
      author={Olaf Ronneberger and Philipp Fischer and Thomas Brox},
      year={2015},
      eprint={1505.04597},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@misc{loshchilov2019decoupled,
      title={Decoupled Weight Decay Regularization}, 
      author={Ilya Loshchilov and Frank Hutter},
      year={2019},
      eprint={1711.05101},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@misc{marius,
    author = {Marius Giger},
    title = {{Unsupervised Anomaly Detection
with Variational Autoencoders in
Heliophysics}},
    year = {2022},
    publisher = {GitHub},
    journal = {GitHub repository},
    howpublished = {\url{https://github.com/i4Ds/sdo-cli}}
}

@misc{zimmerer2018contextencoding,
      title={Context-encoding Variational Autoencoder for Unsupervised Anomaly Detection}, 
      author={David Zimmerer and Simon A. A. Kohl and Jens Petersen and Fabian Isensee and Klaus H. Maier-Hein},
      year={2018},
      eprint={1812.05941},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@incollection{pytorch,
title = {PyTorch: An Imperative Style, High-Performance Deep Learning Library},
author = {Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and Desmaison, Alban and Kopf, Andreas and Yang, Edward and DeVito, Zachary and Raison, Martin and Tejani, Alykhan and Chilamkurthy, Sasank and Steiner, Benoit and Fang, Lu and Bai, Junjie and Chintala, Soumith},
booktitle = {Advances in Neural Information Processing Systems 32},
pages = {8024--8035},
year = {2019},
publisher = {Curran Associates, Inc.},
url = {}
}

@article{vanDerMaaten2008,
  added-at = {2015-06-19T12:07:15.000+0200},
  author = {van der Maaten, Laurens and Hinton, Geoffrey},
  biburl = {https://www.bibsonomy.org/bibtex/28b9aebb404ad4a4c6a436ea413550b30/lopusz_kdd},
  interhash = {370ba8b9e1909b61880a6f47c93bcd49},
  intrahash = {8b9aebb404ad4a4c6a436ea413550b30},
  journal = {Journal of Machine Learning Research},
  keywords = {dimensionality_reduction tSNE visualization},
  pages = {2579--2605},
  timestamp = {2015-08-19T15:19:11.000+0200},
  title = {Visualizing Data using {t-SNE} },
  url = {http://www.jmlr.org/papers/v9/vandermaaten08a.html},
  volume = 9,
  year = 2008
}

@inproceedings{sklearn_api,
  author    = {Lars Buitinck and Gilles Louppe and Mathieu Blondel and
               Fabian Pedregosa and Andreas Mueller and Olivier Grisel and
               Vlad Niculae and Peter Prettenhofer and Alexandre Gramfort
               and Jaques Grobler and Robert Layton and Jake VanderPlas and
               Arnaud Joly and Brian Holt and Ga{\"{e}}l Varoquaux},
  title     = {{API} design for machine learning software: experiences from the scikit-learn
               project},
  booktitle = {ECML PKDD Workshop: Languages for Data Mining and Machine Learning},
  year      = {2013},
  pages = {108--122},
}

@inproceedings{parmar2021cleanfid,
  title={On Aliased Resizing and Surprising Subtleties in GAN Evaluation},
  author={Parmar, Gaurav and Zhang, Richard and Zhu, Jun-Yan},
  booktitle={CVPR},
  year={2022}
}

@misc{radford2021learning,
      title={Learning Transferable Visual Models From Natural Language Supervision}, 
      author={Alec Radford and Jong Wook Kim and Chris Hallacy and Aditya Ramesh and Gabriel Goh and Sandhini Agarwal and Girish Sastry and Amanda Askell and Pamela Mishkin and Jack Clark and Gretchen Krueger and Ilya Sutskever},
      year={2021},
      eprint={2103.00020},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@misc{karras2020training,
      title={Training Generative Adversarial Networks with Limited Data}, 
      author={Tero Karras and Miika Aittala and Janne Hellsten and Samuli Laine and Jaakko Lehtinen and Timo Aila},
      year={2020},
      eprint={2006.06676},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@misc{touvron2021training,
      title={Training data-efficient image transformers & distillation through attention}, 
      author={Hugo Touvron and Matthieu Cord and Matthijs Douze and Francisco Massa and Alexandre Sablayrolles and Hervé Jégou},
      year={2021},
      eprint={2012.12877},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@misc{somepalli2022diffusion,
      title={Diffusion Art or Digital Forgery? Investigating Data Replication in Diffusion Models}, 
      author={Gowthami Somepalli and Vasu Singla and Micah Goldblum and Jonas Geiping and Tom Goldstein},
      year={2022},
      eprint={2212.03860},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@misc{saharia2022palette,
      title={Palette: Image-to-Image Diffusion Models}, 
      author={Chitwan Saharia and William Chan and Huiwen Chang and Chris A. Lee and Jonathan Ho and Tim Salimans and David J. Fleet and Mohammad Norouzi},
      year={2022},
      eprint={2111.05826},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@ARTICLE{10.3389/fspas.2020.00034,
  
AUTHOR={Love, Teri and Neukirch, Thomas and Parnell, Clare E.},   
	 
TITLE={Analyzing AIA Flare Observations Using Convolutional Neural Networks},      
	
JOURNAL={Frontiers in Astronomy and Space Sciences},      
	
VOLUME={7},           
	
YEAR={2020},      
	  
URL={https://www.frontiersin.org/articles/10.3389/fspas.2020.00034},       
	
DOI={10.3389/fspas.2020.00034},      
	
ISSN={2296-987X},   
   
ABSTRACT={In order to efficiently analyse the vast amount of data generated by solar space missions and ground-based instruments, modern machine learning techniques such as decision trees, support vector machines (SVMs) and neural networks can be very useful. In this paper we present initial results from using a convolutional neural network (CNN) to analyse observations from the Atmospheric Imaging Assembly (AIA) in the 1,600Å wavelength. The data is pre-processed to locate flaring regions where flare ribbons are visible in the observations. The CNN is created and trained to automatically analyse the shape and position of the flare ribbons, by identifying whether each image belongs into one of four classes: two-ribbon flare, compact/circular ribbon flare, limb flare, or quiet Sun, with the final class acting as a control for any data included in the training or test sets where flaring regions are not present. The network created can classify flare ribbon observations into any of the four classes with a final accuracy of 94\%. Initial results show that most of the images are correctly classified with the compact flare class being the only class where accuracy drops below 90\% and some observations are wrongly classified as belonging to the limb class.}
}

@Article{angeo-39-861-2021,
AUTHOR = {Innocenti, M. E. and Amaya, J. and Raeder, J. and Dupuis, R. and Ferdousi, B. and Lapenta, G.},
TITLE = {Unsupervised classification of simulated magnetospheric regions},
JOURNAL = {Annales Geophysicae},
VOLUME = {39},
YEAR = {2021},
NUMBER = {5},
PAGES = {861--881},
URL = {https://angeo.copernicus.org/articles/39/861/2021/},
DOI = {10.5194/angeo-39-861-2021}
}

@article{Armstrong2019,
author = {Armstrong, John and Fletcher, Lyndsay},
year = {2019},
month = {06},
pages = {},
title = {Fast Solar Image Classification Using Deep Learning and Its Importance for Automation in Solar Physics},
volume = {294},
journal = {Solar Physics},
doi = {10.1007/s11207-019-1473-z}
}

@article{redmon2018september,
  title={September 2017's Geoeffective Space Weather and Impacts to Caribbean Radio Communications During Hurricane Response},
  author={Redmon, R. J. and Seaton, D. B. and Steenburgh, R. and He, J. and Rodriguez, J. V.},
  journal={Space Weather-the International Journal of Research and Applications},
  volume={16},
  number={9},
  pages={1190--1201},
  year={2018},
  publisher={American Geophysical Union},
  doi={10.1029/2018sw001897}
}

@misc{xu2022characteristics,
      title={Characteristics of Flight Delays during Solar Flares}, 
      author={X. H. Xu and Y. Wang and F. S. Wei and X. S. Feng and M. H. Bo and H. W. Tang and D. S. Wang and L. Bian and B. Y. Wang and W. Y. Zhang and Y. S. Huang and Z. Li and J. P. Guo and P. B. Zuo and C. W. Jiang and X. J. Xu and Z. L. Zhou and P. Zou},
      year={2022},
      eprint={2209.07701},
      archivePrefix={arXiv},
      primaryClass={astro-ph.SR}
}

@article{knipp2016,
author = {Knipp, D. J. and Ramsay, A. C. and Beard, E. D. and Boright, A. L. and Cade, W. B. and Hewins, I. M. and McFadden, R. H. and Denig, W. F. and Kilcommons, L. M. and Shea, M. A. and Smart, D. F.},
title = {The May 1967 great storm and radio disruption event: Extreme space weather and extraordinary responses},
journal = {Space Weather},
volume = {14},
number = {9},
pages = {614-633},
keywords = {solar radio bursts, space weather superstorm, space weather impacts},
doi = {https://doi.org/10.1002/2016SW001423},
url = {https://agupubs.onlinelibrary.wiley.com/doi/abs/10.1002/2016SW001423},
eprint = {https://agupubs.onlinelibrary.wiley.com/doi/pdf/10.1002/2016SW001423},
abstract = {Abstract Although listed as one of the most significant events of the last 80 years, the space weather storm of late May 1967 has been of mostly fading academic interest. The storm made its initial mark with a colossal solar radio burst causing radio interference at frequencies between 0.01 and 9.0 GHz and near-simultaneous disruptions of dayside radio communication by intense fluxes of ionizing solar X-rays. Aspects of military control and communication were immediately challenged. Within hours a solar energetic particle event disrupted high-frequency communication in the polar cap. Subsequently, record-setting geomagnetic and ionospheric storms compounded the disruptions. We explain how the May 1967 storm was nearly one with ultimate societal impact, were it not for the nascent efforts of the United States Air Force in expanding its terrestrial weather monitoring-analysis-warning-prediction efforts into the realm of space weather forecasting. An important and long-lasting outcome of this storm was more formal Department of Defense-support for current-day space weather forecasting. This story develops during the rapid rise of solar cycle 20 and the intense Cold War in the latter half of the twentieth century. We detail the events of late May 1967 in the intersecting categories of solar-terrestrial interactions and the political-military backdrop of the Cold War. This was one of the “Great Storms” of the twentieth century, despite the apparent lack of large geomagnetically induced currents. Radio disruptions like those discussed here warrant the attention of today's radio-reliant, cellular-phone and satellite-navigation enabled world.},
year = {2016}
}

@article{Smith_2007,
	doi = {10.1029/2006sw000300},
  
	url = {https://doi.org/10.1029%2F2006sw000300},
  
	year = 2007,
	month = {jun},
  
	publisher = {American Geophysical Union ({AGU})},
  
	volume = {5},
  
	number = {6},
  
	pages = {n/a--n/a},
  
	author = {David S. Smith and John M. Scalo},
  
	title = {Risks due to X-ray flares during astronaut extravehicular activity},
  
	journal = {Space Weather}
}

@inproceedings{Fargion_2019,
	doi = {10.1142/9789811204296_0025},
  
	url = {https://doi.org/10.1142%2F9789811204296_0025},
  
	year = 2019,
	month = {may},
  
	publisher = {{WORLD} {SCIENTIFIC}
},
  
	author = {Daniele Fargion and Pietro Oliva and P. G. De Sanctis Lucentini and Silvia Pietroni and Fabio La Monaca and Paolo Paggi and Emanuele Habib and Maxim Yu. Khlopov},
  
	title = {Solar neutrino flare, megaton neutrino detectors and human space journey},
  
	booktitle = {Solar Neutrinos}
}

@misc{gopalswamy2023solar,
      title={The Solar Cause of the 2022 February 3 Geomagnetic Storm that Led to the Demise of the Starlink Satellites}, 
      author={Nat Gopalswamy and Hong Xie and Seiji Yashiro and Sachiko Akiyama},
      year={2023},
      eprint={2303.02330},
      archivePrefix={arXiv},
      primaryClass={astro-ph.SR}
}

@article{Cicogna_2021,
	doi = {10.3847/1538-4357/abfafb},
  
	url = {https://doi.org/10.3847%2F1538-4357%2Fabfafb},
  
	year = 2021,
	month = {jul},
  
	publisher = {American Astronomical Society},
  
	volume = {915},
  
	number = {1},
  
	pages = {38},
  
	author = {Domenico Cicogna and Francesco Berrilli and Daniele Calchetti and Dario Del Moro and Luca Giovannelli and Federico Benvenuto and Cristina Campi and Sabrina Guastavino and Michele Piana},
  
	title = {Flare-forecasting Algorithms Based on High-gradient Polarity Inversion Lines in Active Regions},
  
	journal = {The Astrophysical Journal}
}

@misc{guastavino2022operational,
      title={Operational solar flare forecasting via video-based deep learning}, 
      author={Sabrina Guastavino and Francesco Marchetti and Federico Benvenuto and Cristina Campi and Michele Piana},
      year={2022},
      eprint={2209.05128},
      archivePrefix={arXiv},
      primaryClass={astro-ph.SR}
}

@misc{tlatov2023groundbased,
      title={Ground-based Solar Observations for Space Weather Forecasting}, 
      author={A. G. Tlatov and A. A. Pevtsov},
      year={2023},
      eprint={2303.01708},
      archivePrefix={arXiv},
      primaryClass={astro-ph.SR}
}

@article{Aschwanden_2012,
	doi = {10.1088/0004-637x/754/2/112},
  
	url = {https://doi.org/10.1088%2F0004-637x%2F754%2F2%2F112},
  
	year = 2012,
	month = {jul},
  
	publisher = {American Astronomical Society},
  
	volume = {754},
  
	number = {2},
  
	pages = {112},
  
	author = {Markus J. Aschwanden and Samuel L. Freeland},
  
	title = {{AUTOMATED} {SOLAR} {FLARE} {STATISTICS} {IN} {SOFT} X-{RAYS} {OVER} 37 {YEARS} {OF}$\less$i$\greater${GOES}$\less$/i$\greater${OBSERVATIONS}: {THE} {INVARIANCE} {OF} {SELF}-{ORGANIZED} {CRITICALITY} {DURING} {THREE} {SOLAR} {CYCLES}
},
  
	journal = {The Astrophysical Journal}
}

@ARTICLE{imbdataset,
       author = {{Wan}, Jie and {Fu}, Jun-Feng and {Liu}, Jin-Fu and {Shi}, Jia-Kui and {Jin}, Cheng-Gang and {Zhang}, Huai-Peng},
        title = "{Class imbalance problem in short-term solar flare prediction}",
      journal = {Research in Astronomy and Astrophysics},
     keywords = {The Sun, Sun: X-rays, gamma rays, Sun: sunspots, Sun: magnetic fields, Sun: flares, methods: data analysis},
         year = 2021,
        month = nov,
       volume = {21},
       number = {9},
          eid = {237},
        pages = {237},
          doi = {10.1088/1674-4527/21/9/237},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021RAA....21..237W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Liu_2022,
	doi = {10.1002/essoar.10510080.1},
	url = {https://doi.org/10.1002%2Fessoar.10510080.1},
	year = 2022,
	month = {jan},
	publisher = {Wiley},
	author = {Allison Liu and Wendy Carande},
	title = {Data Augmentation of Magnetograms for Solar Flare Prediction using Generative Adversarial Networks}
}

@ARTICLE{deng2021,
       author = {{Deng}, Junlan and {Song}, Wei and {Liu}, Dan and {Li}, Qin and {Lin}, Ganghua and {Wang}, Haimin},
        title = "{Improving the Spatial Resolution of Solar Images Using Generative Adversarial Network and Self-attention Mechanism}",
      journal = {\apj},
     keywords = {1518, 1933, 1974},
         year = 2021,
        month = dec,
       volume = {923},
       number = {1},
          eid = {76},
        pages = {76},
          doi = {10.3847/1538-4357/ac2aa2},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...923...76D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@misc{dash2021high,
      title={High Resolution Solar Image Generation using Generative Adversarial Networks}, 
      author={Ankan Dash and Junyi Ye and Guiling Wang},
      year={2021},
      eprint={2106.03814},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@article{Salvatelli_2022,
	doi = {10.3847/1538-4357/ac867b},
  
	url = {https://doi.org/10.3847%2F1538-4357%2Fac867b},
  
	year = 2022,
	month = {oct},
  
	publisher = {American Astronomical Society},
  
	volume = {937},
  
	number = {2},
  
	pages = {100},
  
	author = {Valentina Salvatelli and Luiz F. G. dos Santos and Souvik Bose and Brad Neuberg and Mark C. M. Cheung and Miho Janvier and Meng Jin and Yarin Gal and Atilim Güne{\c{s}
} Baydin},
  
	title = {Exploring the Limits of Synthetic Creation of Solar {EUV} Images via Image-to-image Translation},
  
	journal = {The Astrophysical Journal}
}

@misc{dhariwal2021diffusion,
      title={Diffusion Models Beat GANs on Image Synthesis}, 
      author={Prafulla Dhariwal and Alex Nichol},
      year={2021},
      eprint={2105.05233},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@misc{vaswani2017attention,
      title={Attention Is All You Need}, 
      author={Ashish Vaswani and Noam Shazeer and Niki Parmar and Jakob Uszkoreit and Llion Jones and Aidan N. Gomez and Lukasz Kaiser and Illia Polosukhin},
      year={2017},
      eprint={1706.03762},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@article{Hurlburt2010,
	doi = {10.1007/s11207-010-9624-2},
  
	url = {https://doi.org/10.1007%2Fs11207-010-9624-2},
  
	year = 2010,
	month = {dec},
  
	publisher = {Springer Science and Business Media {LLC}
},
  
	volume = {275},
  
	number = {1-2},
  
	pages = {67--78},
  
	author = {N. Hurlburt and M. Cheung and C. Schrijver and L. Chang and S. Freeland and S. Green and C. Heck and A. Jaffey and A. Kobashi and D. Schiff and J. Serafin and R. Seguin and G. Slater and A. Somani and R. Timmons},
  
	title = {Heliophysics Event Knowledgebase for~the~Solar Dynamics Observatory ({SDO}) and Beyond},
  
	journal = {Solar Physics}
}

@misc{um2023dont,
      title={Don't Play Favorites: Minority Guidance for Diffusion Models}, 
      author={Soobin Um and Jong Chul Ye},
      year={2023},
      eprint={2301.12334},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@misc{huy2023denoising,
      title={Denoising Diffusion Medical Models}, 
      author={Pham Ngoc Huy and Tran Minh Quan},
      year={2023},
      eprint={2304.09383},
      archivePrefix={arXiv},
      primaryClass={eess.IV}
}

@misc{karchev2022stronglensing,
      title={Strong-Lensing Source Reconstruction with Denoising Diffusion Restoration Models}, 
      author={Konstantin Karchev and Noemi Anau Montel and Adam Coogan and Christoph Weniger},
      year={2022},
      eprint={2211.04365},
      archivePrefix={arXiv},
      primaryClass={astro-ph.IM}
}

@Article{slavaolga,
AUTHOR = {Voloshynovskiy, Slava and Taran, Olga and Kondah, Mouad and Holotyak, Taras and Rezende, Danilo},
TITLE = {Variational Information Bottleneck for Semi-Supervised Classification},
JOURNAL = {Entropy},
VOLUME = {22},
YEAR = {2020},
NUMBER = {9},
ARTICLE-NUMBER = {943},
URL = {https://www.mdpi.com/1099-4300/22/9/943},
PubMedID = {33286710},
ISSN = {1099-4300},
ABSTRACT = {In this paper, we consider an information bottleneck (IB) framework for semi-supervised classification with several families of priors on latent space representation. We apply a variational decomposition of mutual information terms of IB. Using this decomposition we perform an analysis of several regularizers and practically demonstrate an impact of different components of variational model on the classification accuracy. We propose a new formulation of semi-supervised IB with hand crafted and learnable priors and link it to the previous methods such as semi-supervised versions of VAE (M1 + M2), AAE, CatGAN, etc. We show that the resulting model allows better understand the role of various previously proposed regularizers in semi-supervised classification task in the light of IB framework. The proposed IB semi-supervised model with hand-crafted and learnable priors is experimentally validated on MNIST under different amount of labeled data.},
DOI = {10.3390/e22090943}
}

@misc{zimmermann2021scorebased,
      title={Score-Based Generative Classifiers}, 
      author={Roland S. Zimmermann and Lukas Schott and Yang Song and Benjamin A. Dunn and David A. Klindt},
      year={2021},
      eprint={2110.00473},
      archivePrefix={arXiv},
      primaryClass={stat.ML}
}

@misc{wolleb2022diffusion,
      title={Diffusion Models for Medical Anomaly Detection}, 
      author={Julia Wolleb and Florentin Bieder and Robin Sandkühler and Philippe C. Cattin},
      year={2022},
      eprint={2203.04306},
      archivePrefix={arXiv},
      primaryClass={eess.IV}
}

@misc{rombach2022highresolution,
      title={High-Resolution Image Synthesis with Latent Diffusion Models}, 
      author={Robin Rombach and Andreas Blattmann and Dominik Lorenz and Patrick Esser and Björn Ommer},
      year={2022},
      eprint={2112.10752},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@article{Chen2022,
    author = {Chen, Yang and Kempton, Dustin J. and Ahmadzadeh, Azim and Wen, Junzhi and Ji, Anli and Angryk, Rafal A.},
    title = {CGAN-based synthetic multivariate time-series generation: a solution to data scarcity in solar flare forecasting},
    journal = {Neural Computing and Applications},
    year = {2022},
    volume = {34},
    number = {16},
    pages = {13339--13353},
    doi = {10.1007/s00521-022-07361-8},
    url = {https://doi.org/10.1007/s00521-022-07361-8},
    abstract = {One of the major bottlenecks in refining supervised algorithms is data scarcity. This might be caused by a number of reasons often rooted in extremely expensive and lengthy data collection processes. In natural domains such as Heliophysics, it may take decades for sufficiently large samples for machine learning purposes. Inspired by the massive success of generative adversarial networks (GANs) in generating synthetic images, in this study we employed the conditional GAN (CGAN) on a recently released benchmark dataset tailored for solar flare forecasting. Our goal is to generate synthetic multivariate time-series data that (1) are statistically similar to the real data and (2) improve the performance of flare prediction when used to remedy the scarcity of strong flares. To evaluate the generated samples, first, we used the Kullback–Leibler divergence and adversarial accuracy measures to quantify the similarity between the real and synthetic data in terms of their descriptive statistics. Second, we evaluated the impact of the generated samples by training a predictive model on their descriptive statistics, which resulted in a significant improvement (over 1100% in TSS and 350% in HSS). Third, we used the generated time series to examine their high-dimensional contribution to mitigating the scarcity of the strong flares, which we also observed a significant improvement in terms of TSS (4%, 7%, and 31%) and HSS (75%, 35%, and 72%), compared to oversampling, undersampling, and synthetic oversampling methods, respectively. We believe our findings can open new doors toward more robust and accurate flare forecasting models.}
}

@article{refId0,
	author = {{Battaglia, Andrea Francesco} and {Wang, Wen} and {Saqri, Jonas} and {Podladchikova, Tatiana} and {Veronig, Astrid M.} and {Collier, Hannah} and {Dickson, Ewan C. M.} and {Podladchikova, Olena} and {Monstein, Christian} and {Warmuth, Alexander} and {Schuller, Fr\'ed\'eric} and {Harra, Louise} and {Krucker, S\"am}},
	title = {Identifying the energy release site in a solar microflare with a jet},
	DOI= "10.1051/0004-6361/202244996",
	url= "https://doi.org/10.1051/0004-6361/202244996",
	journal = {A\&A},
	year = 2023,
	volume = 670,
	pages = "A56",
}

@article{Huwyler_2022,
	doi = {10.1016/j.ascom.2022.100668},
  
	url = {https://doi.org/10.1016%2Fj.ascom.2022.100668},
  
	year = 2022,
	month = {oct},
  
	publisher = {Elsevier {BV}
},
  
	volume = {41},
  
	pages = {100668},
  
	author = {C. Huwyler and M. Melchior},
  
	title = {Using multiple instance learning for explainable solar flare prediction},
  
	journal = {Astronomy and Computing}
}

@article{Collier_2023,
	doi = {10.1051/0004-6361/202245293},
  
	url = {https://doi.org/10.1051%2F0004-6361%2F202245293},
  
	year = 2023,
	month = {mar},
  
	publisher = {{EDP} Sciences},
  
	volume = {671},
  
	pages = {A79},
  
	author = {Hannah Collier and Laura A. Hayes and Andrea F. Battaglia and Louise K. Harra and Säm Krucker},
  
	title = {Characterising fast-time variations in the hard X-ray time profiles of solar flares using Solar Orbiter's {STIX}
},
  
	journal = {Astronomy {\&}amp$\mathsemicolon$ Astrophysics}
}

@article{YANG2023100409,
title = {An Improved CycleGAN for Data Augmentation in Person Re-Identification},
journal = {Big Data Research},
volume = {34},
pages = {100409},
year = {2023},
issn = {2214-5796},
doi = {https://doi.org/10.1016/j.bdr.2023.100409},
url = {https://www.sciencedirect.com/science/article/pii/S2214579623000424},
author = {Zhenzhen Yang and Jing Shao and Yongpeng Yang},
keywords = {Person re-identification, Cycle-consistent generative adversarial network, Data augmentation, Multi-pseudo regularized label, Semi-supervised learning},
abstract = {Person re-identification (ReID) has attracted more and more attention, which is to retrieve interested persons across multiple non-overlapping cameras. Matching the same person between different camera styles has always been an enormous challenge. In the existing work, cross-camera styles images generated by the cycle-consistent generative adversarial network (CycleGAN) only transfer the camera resolution and ambient lighting. The generated images produce considerable redundancy and inappropriate pictures at the same time. Although the data is added to prevent over-fitting, it also makes significant noise, so the accuracy is not significantly improved. In this paper, an improved CycleGAN is proposed to generate images for achieving improved data augmentation. The transfer of pedestrian posture is added at the same time as transferring the image style. It not only increases the diversity of pedestrian posture but also reduces the domain gap caused by the style change between cameras. Besides, through the multi-pseudo regularized label (MpRL), the generated images are assigned virtual tags dynamically in training. Through many experimental evaluations, we have achieved a very high identification accuracy on Market-1501, DukeMTMC-reID, and CUHK03-NP datasets. On the three datasets, the quantitative results of mAP are 96.20%, 93.72%, and 86.65%, and the quantitative results of rank-1 are 98.27%, 95.37%, and 90.71%, respectively. The experimental results fully show the superiority of our proposed method.}
}

@inbook{Pandey_2023,
   title={Explainable Deep Learning-Based Solar Flare Prediction with Post Hoc Attention for Operational Forecasting},
   ISBN={9783031452758},
   ISSN={1611-3349},
   url={http://dx.doi.org/10.1007/978-3-031-45275-8_38},
   DOI={10.1007/978-3-031-45275-8_38},
   booktitle={Lecture Notes in Computer Science},
   publisher={Springer Nature Switzerland},
   author={Pandey, Chetraj and Angryk, Rafal A. and Georgoulis, Manolis K. and Aydin, Berkay},
   year={2023},
   pages={567–581} }

@article{Huang_2018,
doi = {10.3847/1538-4357/aaae00},
url = {https://dx.doi.org/10.3847/1538-4357/aaae00},
year = {2018},
month = {mar},
publisher = {The American Astronomical Society},
volume = {856},
number = {1},
pages = {7},
author = {Xin Huang and Huaning Wang and Long Xu and Jinfu Liu and Rong Li and Xinghua Dai},
title = {Deep Learning Based Solar Flare Forecasting Model. I. Results for Line-of-sight Magnetograms},
journal = {The Astrophysical Journal},
abstract = {Solar flares originate from the release of the energy stored in the magnetic field of solar active regions, the triggering mechanism for these flares, however, remains unknown. For this reason, the conventional solar flare forecast is essentially based on the statistic relationship between solar flares and measures extracted from observational data. In the current work, the deep learning method is applied to set up the solar flare forecasting model, in which forecasting patterns can be learned from line-of-sight magnetograms of solar active regions. In order to obtain a large amount of observational data to train the forecasting model and test its performance, a data set is created from line-of-sight magnetogarms of active regions observed by SOHO/MDI and SDO/HMI from 1996 April to 2015 October and corresponding soft X-ray solar flares observed by GOES. The testing results of the forecasting model indicate that (1) the forecasting patterns can be automatically reached with the MDI data and they can also be applied to the HMI data; furthermore, these forecasting patterns are robust to the noise in the observational data; (2) the performance of the deep learning forecasting model is not sensitive to the given forecasting periods (6, 12, 24, or 48 hr); (3) the performance of the proposed forecasting model is comparable to that of the state-of-the-art flare forecasting models, even if the duration of the total magnetograms continuously spans 19.5 years. Case analyses demonstrate that the deep learning based solar flare forecasting model pays attention to areas with the magnetic polarity-inversion line or the strong magnetic field in magnetograms of active regions.}
}

@article{Li_2020,
doi = {10.3847/1538-4357/ab6d04},
url = {https://dx.doi.org/10.3847/1538-4357/ab6d04},
year = {2020},
month = {feb},
publisher = {The American Astronomical Society},
volume = {891},
number = {1},
pages = {10},
author = {Xuebao Li and Yanfang Zheng and Xinshuo Wang and Lulu Wang},
title = {Predicting Solar Flares Using a Novel Deep Convolutional Neural Network},
journal = {The Astrophysical Journal},
abstract = {Space weather forecasting is very important, and the prediction of space weather, especially for solar flares, has increasingly attracted research interests with the numerous recent breakthroughs in machine learning. In this study, we propose a novel convolutional neural network (CNN) model to make binary class prediction for both ≥C-class and ≥M-class flares within 24 hr. We collect magnetogram samples of solar active regions (ARs) provided by the Space-weather Helioseismic and Magnetic Imager Active Region Patches (SHARP) data from 2010 May to 2018 September. These samples are used to construct 10 separate data sets. Then, after training, validating, and testing our model, we compare the results of our model with previous studies in several metrics, with a focus on the true skill statistic (TSS). The major results are summarized as follows. (1) We propose a method of shuffle and split cross-validation (CV) based on AR segregation, which is the first attempt to verify the validity and stability of the model in flare prediction. (2) The proposed CNN model achieves a relatively high score of TSS = 0.749 ± 0.079 for ≥M-class prediction, and TSS = 0.679 ± 0.045 for ≥C-class prediction, which is greatly improved compared with previous studies. (3) The model trained on 10 CV data sets is considerably robust and stable in making flare prediction for both ≥C class and ≥M class. Our experimental results indicate that our proposed CNN model is a highly effective method for flare forecasting, with quite excellent prediction performance.}
}

@article{Zheng_2019,
doi = {10.3847/1538-4357/ab46bd},
url = {https://dx.doi.org/10.3847/1538-4357/ab46bd},
year = {2019},
month = {nov},
publisher = {The American Astronomical Society},
volume = {885},
number = {1},
pages = {73},
author = {Yanfang Zheng and Xuebao Li and Xinshuo Wang},
title = {Solar Flare Prediction with the Hybrid Deep Convolutional Neural Network},
journal = {The Astrophysical Journal},
abstract = {We propose a hybrid Convolutional Neural Network (CNN) model (Model 2) and modify a popular CNN model (Model 1) to predict multiclass solar flare occurrence within 24 hr. We collect samples of solar active regions provided by the Space-weather Helioseismic and Magnetic Imager Active Region Patches data from 2010 May to 2018 September. These samples are categorized into four classes (No-flare, C, M, and X), containing 10 separate data sets. Then after training, validating, and testing our models, we compare the results with previous studies in forecast verification metrics with an emphasis on the true skill statistic (TSS). The main results are summarized as follows. (1) This is the first time that the CNN models are used to make multiclass predictions of solar flare. (2) Model 2 has better values of all statistical scores than Model 1 in every class. (3) Model 2 achieves relatively high average scores of TSS = 0.768 for No-flare class, 0.538 for C class, 0.534 for M class, and 0.552 for X class, which are the best results from the existing literatures. (4) Model 2 also can be used to make binary class flare predictions for ≥M-class major flares, and the performance yields a TSS with 0.749 ± 0.079. (5) Model 2 obtains fairly good scores in other metrics for both multiclass flare predictions and ≥M-class major flare predictions. We surmise that some crucial features extracted automatically by our models may have not been excavated before and could provide important clues for studying the mechanism of flare.}
}

@ARTICLE{2023ApJSYi,
       author = {{Yi}, Kangwoo and {Moon}, Yong-Jae and {Jeong}, Hyun-Jin},
        title = "{Application of Deep Reinforcement Learning to Major Solar Flare Forecasting}",
      journal = {\apjs},
     keywords = {Solar flares, Neural networks, The Sun, 1496, 1933, 1693},
         year = 2023,
        month = apr,
       volume = {265},
       number = {2},
          eid = {34},
        pages = {34},
          doi = {10.3847/1538-4365/acb76d},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2023ApJS..265...34Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pandey_2022,
  
AUTHOR={Pandey, Chetraj and Ji, Anli and Angryk, Rafal A. and Georgoulis, Manolis K. and Aydin, Berkay},   
	 
TITLE={Towards coupling full-disk and active region-based flare prediction for operational space weather forecasting},      
	
JOURNAL={Frontiers in Astronomy and Space Sciences},      
	
VOLUME={9},           
	
YEAR={2022},      
	  
URL={https://www.frontiersin.org/articles/10.3389/fspas.2022.897301},       
	
DOI={10.3389/fspas.2022.897301},      
	
ISSN={2296-987X},   
   
ABSTRACT={Solar flare prediction is a central problem in space weather forecasting and has captivated the attention of a wide spectrum of researchers due to recent advances in both remote sensing as well as machine learning and deep learning approaches. The experimental findings based on both machine and deep learning models reveal significant performance improvements for task specific datasets. Along with building models, the practice of deploying such models to production environments under operational settings is a more complex and often time-consuming process which is often not addressed directly in research settings. We present a set of new heuristic approaches to train and deploy an operational solar flare prediction system for ≥M1.0-class flares with two prediction modes: full-disk and active region-based. In full-disk mode, predictions are performed on full-disk line-of-sight magnetograms using deep learning models whereas in active region-based models, predictions are issued for each active region individually using multivariate time series data instances. The outputs from individual active region forecasts and full-disk predictors are combined to a final full-disk prediction result with a meta-model. We utilized an equal weighted average ensemble of two base learners’ flare probabilities as our baseline meta learner and improved the capabilities of our two base learners by training a logistic regression model. The major findings of this study are: 1) We successfully coupled two heterogeneous flare prediction models trained with different datasets and model architecture to predict a full-disk flare probability for next 24 h, 2) Our proposed ensembling model, i.e., logistic regression, improves on the predictive performance of two base learners and the baseline meta learner measured in terms of two widely used metrics True Skill Statistic (TSS) and Heidke Skill Score (HSS), and 3) Our result analysis suggests that the logistic regression-based ensemble (Meta-FP) improves on the full-disk model (base learner) by ∼9% in terms TSS and ∼10% in terms of HSS. Similarly, it improves on the AR-based model (base learner) by ∼17% and ∼20% in terms of TSS and HSS respectively. Finally, when compared to the baseline meta model, it improves on TSS by ∼10% and HSS by ∼15%.}
}
